American postdoctoral salaries do not account for growing disparities in cost of living

The National Institute of Health (NIH) sets postdoctoral (postdoc) trainee stipend levels that many American institutions and investigators use as a basis for postdoc salaries. Although salary standards are held constant across universities, the cost of living in those universities' cities and towns vary widely. Across non-postdoc jobs, more expensive cities pay workers higher wages that scale with an increased cost of living. This work investigates the extent to which postdoc wages account for cost-of-living differences. More than 27,000 postdoc salaries across all US universities are analyzed alongside measures of regional differences in cost of living. We find that postdoc salaries do not account for cost-of-living differences, in contrast with the broader labor market in the same cities and towns. Despite a modest increase in income in high cost of living areas, real (cost of living adjusted) postdoc salaries differ by 29% ($15k 2021 USD) between the least and most expensive areas. Cities that produce greater numbers of tenure-track faculty relative to students such as Boston, New York, and San Francisco are among the most impacted by this pay disparity. The postdoc pay gap is growing and is well-positioned to incur a greater financial burden on economically disadvantaged groups and contribute to faculty hiring disparities in women and racial minorities.

==> trash.tex <==
%Academic funding agencies suggest a maximum postdoc duration of around five years \cite{ferguson2014national}. In the biomedical sciences, the duration of an average postdoc ranges between 4-5 years \cite{kahn2017impact}, slightly less than the 5-7 year probationary period on the tenure track \cite{nerad1999postdoctoral}. 
%Even beyond these training years however, the financial impact of doing a postdoc on salary carries over at least 15 years following PhD completion [2].
%Although the financial impacts of doing a postdoc are long lasting [2], because postdoctoral training is considered a transitory training period rather than a career salary is often disregarded when trainees are  choosing a postdoc. Funding guidelines set by agencies, such as the NIH, set standards for postdoc salaries that are constant across universities. The value of that income can vary greatly across the United States however. Cost of living is not taken into account when setting NIH postdoc salaries which often impose restrictions and limits on universities on how income can be supplemented. An individual's real income measures the actual value of an individual's income in a geographic region [CITE BLS].




Among them, the training institution plays an outsized role in academic career prospects: 25\% of universities produce 71-86\% of all tenure-track faculty hires and only 9-14\% of faulty find positions at universities more prestigious than their doctorate [3].
The same relationship is observed of postdoctoral prestige \cite{mc1982postdoctoral}.
Faculty placements are also increasingly dependent on postdoctoral fellowships and career development awards which are unevenly distributed across institutions [4].




Choices made during the doctoral and postdoctoral periods of training have long lasting impacts on a researcher's career outcomes. 


%For example, doing a postdoc after completing a PhD provides an advantage in finding tenure-track academic positions [1] but results in long-lasting salary reductions if the trainee leaves academia [2].
%The mentorship provided by postdoctoral advisors also plays an large role future career outcomes [5]. 

% First PI grants generally occur 

% bridge why this is relevant
While trainees have some control over the institutions and research environments that they choose to join, postdocs have little or no control over other important factors which impact academic career prospects such as gender \cite{huang2020historical, way2016gender} [6] [9], race [8] [10] , parenthood [9], and socioeconomic roots [7]. 
A goal of many academic institutions is to reduce and remove such systemic inequalities.


%Postdoc salaries are lower in America's most expensive cities. 
%Why would a postdoc choose to work in a university or city with lower wages? 

%To determine the relationship between academic career prospects with postdoctoral wages we use a dataset of \hl{X} TT faculty across \hl{Y} US institutions and the institutions where they recieved their PhDs. Although this dataset relies on PhD training and not postdoc training, prior work has shown that postdoc training institutions are similarly important for academic career prospects. 


\hl{
America's most expensive cities, like New York, San Francisco, and Boston, contain many of the top-ranked universities in the world.  
% Many top ranked American universities are located in high cost of living cities like Boston, New York, and San Francisco. 
% It is possible that these top-ranked universities could be outliers in the level of support that they provide postdocs however, accounting for cost of living. 
We used the CWUR rankings of the top American universities alongside postdoc salaries and RPPs to look at the relationship between university prestige and cost of living and whether top ranked universities are paying enough to offset those differences in cost of living. 
We looked, in particular, at the top 20 ranked universities in this dataset.
We divided the range of RPPs across universities into quadrants, beteen the most expensive region, San Francisco (RPP=\hl{X}), and the least expensive region (RPP=\hl{Y}). 
We observe that top-ranked universities are disproportionately located in the most expensive areas in the US. 
The top 20 schools account for \hl{55\% (n=X/Y)} of universities in the top quadrant, and only \hl{1.5\% (n=X/Y)} of universities in the bottom quadrant. 
Like other universities in higher cost-of-living areas, top tier universities pay higher salaries to their postdocs \hl{[STATS]}. 
Again, however, those higher salaries do not account for differences in cost of living. Of the top 20 universities, only \hl{4} pay a salary above the mean real salary for postdocs (Duke, Johns Hopkins, Penn, and University of Chicago). 
Across universities, the median real salary for a postdoc working in a top 20 universities is \hl{X\% (Y 2021 dollars)} below the median postdoc salary. 
}
To develop an appreciation for how impactful these institutions are on the scientific spandscape we looked at a dataset of faculty hiring data from Clauset et al [X]. Across a survey of Computer Science, History, and Business school hires, PhDs from the top 20 institutions account for \hl{X-Y\%} of total faculty hires. Postdoctoral training institutions play an equal or greater role in faculty hiring than PhD institutions in the biomedical sciences [CITATION]. 

